OPT-R: Exploring the Role of Explanations in Finetuning and Prompting for Reasoning Skills of Large Language Models

In this paper, we conduct a thorough investigation into the reasoning capabilities of Large Language Models (LLMs), focusing specifically on the Open Pretrained Transformers (OPT) models as a representative of such models. Our study entails finetuning three different sizes of OPT on a carefully curated reasoning corpus, resulting in two sets of finetuned models: OPT-R, finetuned without explanations, and OPT-RE, finetuned with explanations. We then evaluate all models on 57 out-of-domain tasks drawn from the SUPER-NATURALINSTRUCTIONS benchmark, covering 26 distinct reasoning skills, utilizing three prompting techniques. Through a comprehensive grid of 27 configurations and 6,156 test evaluations, we investigate the dimensions of finetuning, prompting, and scale to understand the role of explanations on different reasoning skills. Our findings reveal that having explanations in the fewshot exemplar has no significant impact on the model's performance when the model is finetuned, while positively affecting the non-finetuned counterpart. Moreover, we observe a slight yet consistent increase in classification accuracy as we incorporate explanations during prompting and finetuning, respectively. Finally, we offer insights on which skills benefit the most from incorporating explanations during finetuning and prompting, such as Numerical (+20.4%) and Analogical (+13.9%) reasoning, as well as skills that exhibit negligible or negative effects.

==> math_commands.tex <==
%%%%% NEW MATH DEFINITIONS %%%%%

\usepackage{amsmath,amsfonts,bm}

% Mark sections of captions for referring to divisions of figures
\newcommand{\figleft}{{\em (Left)}}
\newcommand{\figcenter}{{\em (Center)}}
\newcommand{\figright}{{\em (Right)}}
\newcommand{\figtop}{{\em (Top)}}
\newcommand{\figbottom}{{\em (Bottom)}}
\newcommand{\captiona}{{\em (a)}}
\newcommand{\captionb}{{\em (b)}}
\newcommand{\captionc}{{\em (c)}}
\newcommand{\captiond}{{\em (d)}}

% Highlight a newly defined term
\newcommand{\newterm}[1]{{\bf #1}}


% Figure reference, lower-case.
\def\figref#1{figure~\ref{#1}}
% Figure reference, capital. For start of sentence
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
% Section reference, lower-case.
\def\secref#1{section~\ref{#1}}
% Section reference, capital.
\def\Secref#1{Section~\ref{#1}}
% Reference to two sections.
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
% Reference to three sections.
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
% Reference to an equation, lower-case.
\def\eqref#1{equation~\ref{#1}}
% Reference to an equation, upper case
\def\Eqref#1{Equation~\ref{#1}}
% A raw reference to an equation---avoid using if possible
\def\plaineqref#1{\ref{#1}}
% Reference to a chapter, lower-case.
\def\chapref#1{chapter~\ref{#1}}
% Reference to an equation, upper case.
\def\Chapref#1{Chapter~\ref{#1}}
% Reference to a range of chapters
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
% Reference to an algorithm, lower-case.
\def\algref#1{algorithm~\ref{#1}}
% Reference to an algorithm, upper case.
\def\Algref#1{Algorithm~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
% Reference to a part, lower case
\def\partref#1{part~\ref{#1}}
% Reference to a part, upper case
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
\def\1{\bm{1}}
\newcommand{\train}{\mathcal{D}}
\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
\newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

\def\eps{{\epsilon}}


% Random variables
\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
% rm is already a command, just don't name any random variables m
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

% Random vectors
\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}

% Elements of random vectors
\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

% Random matrices
\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

% Elements of random matrices
\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

% Vectors
\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vtheta{{\bm{\theta}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}

% Elements of vectors
\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

% Matrix
\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}

% Tensor
\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}


% Graph
\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

% Sets
\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
% Don't use a set called E, because this would be the same as our symbol
% for expectation.
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sZ{{\mathbb{Z}}}

% Entries of a matrix
\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

% entries of a tensor
% Same font as tensor, without \bm wrapper
\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

% The true underlying data generating distribution
\newcommand{\pdata}{p_{\rm{data}}}
% The empirical distribution defined by the training set
\newcommand{\ptrain}{\hat{p}_{\rm{data}}}
\newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
% The model distribution
\newcommand{\pmodel}{p_{\rm{model}}}
\newcommand{\Pmodel}{P_{\rm{model}}}
\newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
% Stochastic autoencoder distributions
\newcommand{\pencode}{p_{\rm{encoder}}}
\newcommand{\pdecode}{p_{\rm{decoder}}}
\newcommand{\precons}{p_{\rm{reconstruct}}}

\newcommand{\laplace}{\mathrm{Laplace}} % Laplace distribution

\newcommand{\E}{\mathbb{E}}
\newcommand{\Ls}{\mathcal{L}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
\newcommand{\rect}{\mathrm{rectifier}}
\newcommand{\softmax}{\mathrm{softmax}}
\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
\newcommand{\KL}{D_{\mathrm{KL}}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\standarderror}{\mathrm{SE}}
\newcommand{\Cov}{\mathrm{Cov}}
% Wolfram Mathworld says $L^2$ is for function spaces and $\ell^2$ is for vectors
% But then they seem to use $L^2$ for vectors throughout the site, and so does
% wikipedia.
\newcommand{\normlzero}{L^0}
\newcommand{\normlone}{L^1}
\newcommand{\normltwo}{L^2}
\newcommand{\normlp}{L^p}
\newcommand{\normmax}{L^\infty}

\newcommand{\parents}{Pa} % See usage in notation.tex. Chosen to match Daphne's book.

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\Tr}{Tr}
\let\ab\allowbreak


==> tables/results.tex <==


\begin{table*}[]
    \centering
\begin{tabular}{@{}lccccccccccc@{}}
\toprule
  & \multicolumn{3}{c}{\textbf{OPT}} &  \phantom{a} & \multicolumn{3}{c}{\textbf{OPT-R}} & \phantom{a} & \multicolumn{3}{c}{\textbf{OPT-RE}} \\
  \cmidrule{2-4} \cmidrule{6-8} \cmidrule{10-12} \\
\textbf{Reasoning Skill} &          \textbf{1.3B} &   \textbf{6.7B} & \textbf{13B} && \textbf{1.3B} & \textbf{6.7B} & \textbf{13B} && \textbf{1.3B} & \textbf{6.7B} & \textbf{13B} \\
\midrule
\textbf{Multihop Reasoning                                } &  41.9 &  29.2 &  24.2 &&  42.6 &  32.1 &  45.0 &&  40.4 &  32.6 &  38.0 \\
\textbf{Temporal Reasoning                                } &  49.6 &  50.6 &  49.0 &&  46.7 &  47.4 &  45.3 &&  34.6 &  42.2 &  38.7 \\
\textbf{Logical Reasoning                                 } &  31.4 &  33.6 &  35.2 &&  33.7 &  33.9 &  34.7 &&  33.8 &  46.0 &  35.3 \\
\textbf{Numerical Reasoning                               } &  65.9 &  44.1 &  39.0 &&  64.7 &  66.0 &  65.2 &&  64.7 &  64.9 &  64.7 \\
\textbf{Grammatical Reasoning                             } &  49.9 &  50.4 &  65.0 &&  62.1 &  55.8 &  61.9 &&  61.9 &  61.9 &  65.4 \\
\textbf{Counting                                          } &  17.4 &  18.6 &  24.0 &&  13.0 &  13.1 &  12.0 &&  28.6 &  33.3 &  36.9 \\
\textbf{Reasoning with Symbols                            } &  50.6 &  48.9 &  42.1 &&  52.5 &  51.1 &  51.7 &&  51.4 &  53.1 &  52.7 \\
\textbf{Social Situations                                 } &  48.2 &  45.9 &  45.6 &&  50.4 &  51.2 &  58.1 &&  50.1 &  51.9 &  55.0 \\
\textbf{Textual Entailment                                } &  40.7 &  40.4 &  44.9 &&  47.4 &  49.7 &  44.9 &&  50.4 &  52.1 &  51.3 \\
\textbf{Analogical Reasoning                              } &  41.2 &  49.5 &  47.8 &&  61.1 &  62.0 &  64.4 &&  59.5 &  60.9 &  62.2 \\
\textbf{Relational Reasoning                              } &  51.0 &  51.2 &  51.0 &&  47.9 &  46.9 &  48.8 &&  42.7 &  46.2 &  44.9 \\
\textbf{Social Interactions                               } &  32.4 &  37.6 &  34.0 &&  39.9 &  39.5 &  47.4 &&  36.5 &  39.8 &  43.6 \\
\textbf{Spatial Reasoning                                 } &  46.4 &  50.0 &  44.9 &&  53.2 &  50.8 &  51.4 &&  37.8 &  47.5 &  62.4 \\
\textbf{Deductive Reasoning                               } &  41.1 &  40.8 &  39.3 &&  38.5 &  40.8 &  41.7 &&  40.4 &  39.5 &  43.3 \\
\textbf{TE - Deductive Reasoning                          } &  33.7 &  41.2 &  40.0 &&  30.2 &  30.5 &  29.6 &&  29.2 &  30.6 &  29.9 \\
\textbf{Argument Reasoning                                } &  60.5 &  59.9 &  59.9 &&  43.0 &  44.2 &  50.6 &&  43.6 &  51.2 &  51.7 \\
\textbf{Reasoning on Objects                              } &  50.0 &  52.9 &  62.4 &&  59.7 &  67.6 &  64.1 &&  60.8 &  64.7 &  53.6 \\
\textbf{Physical Reasoning                                } &  40.7 &  42.5 &  38.5 &&  43.8 &  35.3 &  37.2 &&  49.9 &  51.9 &  48.2 \\
\textbf{Commonsense Reasoning                             } &  29.3 &  30.4 &  35.7 &&  28.5 &  30.2 &  29.8 &&  27.9 &  31.4 &  28.3 \\
\textbf{Scientific Reasoning                              } &  22.3 &  22.8 &  24.9 &&  23.2 &  23.6 &  26.6 &&  25.6 &  23.2 &  24.7 \\
\textbf{Abductive Reasoning                               } &  33.3 &  41.7 &  33.3 &&  34.2 &  35.8 &  33.3 &&  38.3 &  35.8 &  31.7 \\
\textbf{Ethics                                            } &  25.5 &  24.3 &  27.6 &&  26.1 &  24.1 &  27.4 &&  27.8 &  24.8 &  30.0 \\
\textbf{TE - Analogical Reasoning                         } &  16.6 &  20.6 &  18.8 &&  16.1 &  23.7 &  22.3 &&  18.7 &  17.3 &  18.5 \\
\textbf{Causal Reasoning                                  } &  51.8 &  50.0 &  50.0 &&  46.8 &  50.0 &  50.0 &&  51.4 &  50.0 &  50.0 \\
\textbf{Reasoning on Strings                              } &  60.7 &  60.7 &  60.7 &&  62.2 &  60.7 &  60.7 &&  60.7 &  60.7 &  60.7 \\
\textbf{Numerical Commonsense                             } &  59.2 &  59.2 &  59.2 &&  59.2 &  59.2 &  58.7 &&  59.2 &  59.7 &  59.2 \\
\bottomrule
\end{tabular}
\caption{Results}
\label{tab:results-test}
\end{table*}


==> tables/results_model.tex <==
\begin{table*}[]
    \centering
\begin{tabular}{lccc}
\toprule
{} &     \textbf{OPT} &     \textbf{OPT-R} &     \textbf{OPT-RE} \\
\midrule
\textbf{\textit{Skills where OPT-R helps}} \\
\textbf{Numerical Reasoning                               } &  49.7 &  65.3 &  64.8 \\
\textbf{Multihop Reasoning                                } &  31.7 &  39.9 &  37.0 \\
\textbf{Social Situations        } &  46.6 &  53.2 &  52.3 \\
\textbf{Analogical Reasoning                              } &  46.2 &  62.5 &  60.9 \\
\textbf{Social Interactions                  } &  34.7 &  42.3 &  40.0 \\
\textbf{Spatial Reasoning        } &  47.1 &  51.8 &  49.2 \\
\textbf{Reasoning on Objects                              } &  55.1 &  63.8 &  59.7 \\
\textbf{Scientific Reasoning                              } &  23.3 &  24.5 &  24.5 \\
\textbf{TE - Analogical Reasoning        } &  18.7 &  20.7 &  18.1 \\

\quad \textbf{\textit{Skills where OPT-RE further helps}} \\
\textbf{Logical Reasoning                                 } &  33.4 &  34.1 &  38.4 \\
\textbf{Reasoning with Symbols       } &  47.2 &  51.8 &  52.4 \\
\textbf{Textual Entailment                                } &  42.0 &  47.3 &  51.2 \\
\textbf{Grammatical Reasoning                             } &  55.1 &  60.0 &  63.1 \\
\textbf{Ethics                                            } &  25.8 &  25.9 &  27.6 \\
\textbf{Deductive Reasoning                               } &  40.4 &  40.4 &  41.1 \\
\textbf{Reasoning on Strings                              } &  60.7 &  61.2 &  60.7 \\
\textbf{Numerical Commonsense } &  59.2 &  59.0 &  59.4 \\

\midrule
\textbf{\textit{Tasks where OPT-R does not help}} \\
\textbf{Causal Reasoning                                  } &  50.6 &  48.9 &  50.5 \\
\textbf{Temporal Reasoning                                } &  49.7 &  46.5 &  38.5 \\
\textbf{Relational Reasoning                              } &  51.1 &  47.9 &  44.6 \\
\textbf{Counting                           } &  20.0 &  12.7 &  32.9 \\
\textbf{TE - Deductive Reasoning         } &  38.3 &  30.1 &  29.9 \\
\textbf{Argument Reasoning                                } &  60.1 &  45.9 &  48.8 \\
\textbf{Physical Reasoning       } &  40.6 &  38.8 &  50.0 \\
\textbf{Commonsense Reasoning                             } &  31.8 &  29.5 &  29.2 \\
\textbf{Abductive Reasoning                               } &  36.1 &  34.4 &  35.3 \\
\bottomrule
\end{tabular}
\caption{Results (Zhijing: here is a tentative format that we can try. I copied the original one right below so we have a backup.)}
\label{tab:results-test}
\end{table*}


% \begin{table*}[]
%     \centering
% \begin{tabular}{lccc}
% \toprule
% {} &     \textbf{OPT} &     \textbf{OPT-R} &     \textbf{OPT-RE} \\
% \midrule
% \textbf{Multihop Reasoning                                } &  31.7 &  39.9 &  37.0 \\
% \textbf{Temporal Reasoning                                } &  49.7 &  46.5 &  38.5 \\
% \textbf{Logical Reasoning                                 } &  33.4 &  34.1 &  38.4 \\
% \textbf{Numerical Reasoning                               } &  49.7 &  65.3 &  64.8 \\
% \textbf{Grammatical Reasoning                             } &  55.1 &  60.0 &  63.1 \\
% \textbf{Counting                           } &  20.0 &  12.7 &  32.9 \\
% \textbf{Reasoning with Symbols       } &  47.2 &  51.8 &  52.4 \\
% \textbf{Social Situations        } &  46.6 &  53.2 &  52.3 \\
% \textbf{Textual Entailment                                } &  42.0 &  47.3 &  51.2 \\
% \textbf{Analogical Reasoning                              } &  46.2 &  62.5 &  60.9 \\
% \textbf{Relational Reasoning                              } &  51.1 &  47.9 &  44.6 \\
% \textbf{Social Interactions                  } &  34.7 &  42.3 &  40.0 \\
% \textbf{Spatial Reasoning        } &  47.1 &  51.8 &  49.2 \\
% \textbf{Deductive Reasoning                               } &  40.4 &  40.4 &  41.1 \\
% \textbf{TE - Deductive Reasoning         } &  38.3 &  30.1 &  29.9 \\
% \textbf{Argument Reasoning                                } &  60.1 &  45.9 &  48.8 \\
% \textbf{Reasoning on Objects                              } &  55.1 &  63.8 &  59.7 \\
% \textbf{Physical Reasoning       } &  40.6 &  38.8 &  50.0 \\
% \textbf{Commonsense Reasoning                             } &  31.8 &  29.5 &  29.2 \\
% \textbf{Scientific Reasoning                              } &  23.3 &  24.5 &  24.5 \\
% \textbf{Abductive Reasoning                               } &  36.1 &  34.4 &  35.3 \\
% \textbf{Ethics                                            } &  25.8 &  25.9 &  27.6 \\
% \textbf{TE - Analogical Reasoning        } &  18.7 &  20.7 &  18.1 \\
% \textbf{Causal Reasoning                                  } &  50.6 &  48.9 &  50.5 \\
% \textbf{Reasoning on Strings                              } &  60.7 &  61.2 &  60.7 \\
% \textbf{Numerical Commonsense } &  59.2 &  59.0 &  59.4 \\
% \bottomrule
% \end{tabular}
% \caption{Results}
% \label{tab:results-test}
% \end{table*}


==> tables/results_opt_fewshot_e.tex <==
\begin{table}[ht!]
\centering
\begin{tabular}{lccc}
\toprule
\textbf{Skill} &     \textbf{OPT} &     \textbf{OPT-R} &     \textbf{OPT-RE} \\ % Delta(OPT, min(OPT-R, OPT-RE))
\midrule
\textbf{Argument       } &  60.1 &  45.9 &  48.8 \\ % 14.2
\textbf{Temporal       } &  49.7 &  46.5 &  38.5 \\ % 11.2
\textbf{TE - Deductive } &  38.3 &  30.1 &  29.9 \\ % 8.4
\textbf{Relational     } &  51.1 &  47.9 &  44.6 \\ % 6.5
\textbf{Commonsense    } &  31.8 &  29.5 &  29.2 \\ % 2.6
\textbf{Causal         } &  50.6 &  48.9 &  50.5 \\ % 1.7
\textbf{Abductive      } &  36.1 &  34.4 &  35.3 \\ % 1.7
\bottomrule
\end{tabular}
\caption{Reasoning skills where \ourmodel{R} models performs worse than OPT using Fewshot-E prompting across scale and tasks. TE is Textual Entailment.}
\label{tab:results-opt-re}
\end{table}


==> tables/results_opt_r_fewshot.tex <==
\begin{table}[ht!]
\centering
\begin{tabular}{lccc}
\toprule
\textbf{Skill} &     \textbf{OPT} &     \textbf{OPT-R} &     \textbf{OPT-RE} \\
\midrule
\textbf{Numerical           } &  39.9 &  65.1 &  64.7 \\
\textbf{Analogical          } &  51.9 &  63.3 &  60.7 \\
\textbf{Soc Interactions    } &  33.6 &  43.8 &  40.2 \\
\textbf{Objects             } &  53.5 &  61.4 &  60.0 \\
\textbf{Soc Situations      } &  46.3 &  53.2 &  51.9 \\
\textbf{Spatial             } &  44.1 &  49.8 &  49.6 \\
\textbf{Abductive           } &  33.9 &  36.9 &  34.2 \\
\textbf{Strings             } &  60.7 &  61.1 &  60.7 \\
\textbf{Relational          } &  47.4 &  47.6 &  44.8 \\
\bottomrule
\end{tabular}
\caption{Reasoning skills where \ourmodel{R} performs best using Fewshot prompting across scale and tasks. Soc is Social. TE is Textual Entailment.}
\label{tab:results-opt-r-fewshot}
\end{table}



==> tables/results_opt_r_fewshot_e.tex <==
\begin{table}[ht!]
\centering
\begin{tabular}{lccc}
\toprule
\textbf{Skill} &     \textbf{OPT} &     \textbf{OPT-R} &     \textbf{OPT-RE} \\
\midrule
\textbf{Analogical          } &  46.2 &  62.5 &  60.9 \\ % 16.3
\textbf{Numerical           } &  49.7 &  65.3 &  64.8 \\ % 15.6
\textbf{Objects             } &  55.1 &  63.8 &  59.7 \\ % 8.7
\textbf{Multihop            } &  31.7 &  39.9 &  37.0 \\ % 8.2
\textbf{Soc Interactions    } &  34.7 &  42.3 &  40.0 \\ % 7.6
\textbf{Soc Situations      } &  46.6 &  53.2 &  52.3 \\ % 6.6
\textbf{Spatial             } &  47.1 &  51.8 &  49.2 \\ % 4.7
\textbf{TE - Analogical     } &  18.7 &  20.7 &  18.1 \\ % 2.0
\textbf{Strings             } &  60.7 &  61.2 &  60.7 \\ % 0.5
\bottomrule
\end{tabular}
\caption{Reasoning skills where \ourmodel{R} performs best using Fewshot-E prompting across scale and tasks. Soc is Social. TE is Textual Entailment.}
\label{tab:results-opt-r}
\end{table}


==> tables/results_opt_re_fewshot.tex <==
\begin{table}[ht!]
\centering
\begin{tabular}{lccc}
\toprule
\textbf{Skill} &     \textbf{OPT} &     \textbf{OPT-R} &     \textbf{OPT-RE} \\ % Delta(OPT-RE, OPT)
\midrule
\textbf{Physical         } &  35.8 &  36.9 &  48.1 \\
\textbf{Counting         } &  19.6 &  13.5 &  29.8 \\
\textbf{Entailment       } &  43.3 &  47.1 &  51.9 \\
\textbf{Symbols          } &  44.2 &  51.7 &  51.9 \\
\textbf{Grammatical      } &  54.4 &  61.2 &  62.0 \\
\textbf{Logical          } &  31.7 &  33.7 &  36.9 \\
\textbf{Multihop         } &  36.6 &  38.9 &  39.5 \\
\textbf{TE - Analogical  } &  16.3 &  18.6 &  18.7 \\
\textbf{Scientific       } &  23.4 &  24.3 &  25.0 \\
\textbf{Deductive        } &  39.4 &  39.4 &  40.0 \\
\bottomrule
\end{tabular}
\caption{Reasoning skills where \ourmodel{RE} performs best using Fewshot prompting across scale and tasks. TE is Textual Entailment.}
\label{tab:results-opt-re-fewshot}
\end{table}


==> tables/results_opt_re_fewshot_e.tex <==
\begin{table}[ht!]
\centering
\begin{tabular}{lccc}
\toprule
\textbf{Skill} &     \textbf{OPT} &     \textbf{OPT-R} &     \textbf{OPT-RE} \\ % Delta(OPT-RE, OPT)
\midrule

\textbf{Counting    } &  20.0 &  12.7 &  32.9 \\ % 12.9
\textbf{Physical    } &  40.6 &  38.8 &  50.0 \\ % 9.4
\textbf{Entailment  } &  42.0 &  47.3 &  51.2 \\ % 9.2
\textbf{Grammatical } &  55.1 &  60.0 &  63.1 \\ % 8
\textbf{Symbols     } &  47.2 &  51.8 &  52.4 \\ % 5.2
\textbf{Logical     } &  33.4 &  34.1 &  38.4 \\ % 5
\textbf{Ethics      } &  25.8 &  25.9 &  27.6 \\ % 1.8
\textbf{Scientific  } &  23.3 &  24.5 &  24.5 \\ % 1.2
\textbf{Reasoning   } &  40.4 &  40.4 &  41.1 \\ % 0.7
\textbf{Numerical CS} &  59.2 &  59.0 &  59.4 \\ % 0.2

\bottomrule
\end{tabular}
\caption{Reasoning skills where \ourmodel{RE} performs best using Fewshot-E prompting across scale and tasks. CS is Commonsense.}
\label{tab:results-opt-re}
\end{table}

